DROID-Splat: Combining end-to-end SLAM with 3D Gaussian Splatting

Recent progress in scene synthesis makes standalone SLAM systems purely based on optimizing hyperprimitives with a Rendering objective possible. However, the tracking performance still lacks behind traditional and end-to-end SLAM systems. An optimal trade-off between robustness, speed and accuracy has not yet been reached, especially for monocular video. In this paper, we introduce a SLAM system based on an end-to-end Tracker and extend it with a Renderer based on recent 3D Gaussian Splatting techniques. Our framework \textbf{DroidSplat} achieves both SotA tracking and rendering results on common SLAM benchmarks. We implemented multiple building blocks of modern SLAM systems to run in parallel, allowing for fast inference on common consumer GPU's. Recent progress in monocular depth prediction and camera calibration allows our system to achieve strong results even on in-the-wild data without known camera intrinsics. Code will be available at \url{https://github.com/ChenHoy/DROID-Splat}.

==> preliminaries.tex <==
We base our system on online end-to-end SLAM \cite{droid}. It consists of multiple modular components, which can be run in parallel: i) a local frontend ii) a global backend iii) a loop detector and iv) a renderer. 
We track the camera by perfor

We follow the reconstruction paradigm of DROID-SLAM \cite{droid}, which uses dense optical flow estimated by a recurrent neural network \cite{raft}. 
